A Survey of Sim-to-Real Methods in RL: Progress, Prospects and Challenges with Foundation Models

Deep Reinforcement Learning (RL) has been explored and verified to be effective in solving decision-making tasks in various domains, such as robotics, transportation, recommender systems, etc. It learns from the interaction with environments and updates the policy using the collected experience. However, due to the limited real-world data and unbearable consequences of taking detrimental actions, the learning of RL policy is mainly restricted within the simulators. This practice guarantees safety in learning but introduces an inevitable sim-to-real gap in terms of deployment, thus causing degraded performance and risks in execution. There are attempts to solve the sim-to-real problems from different domains with various techniques, especially in the era with emerging techniques such as large foundations or language models that have cast light on the sim-to-real. This survey paper, to the best of our knowledge, is the first taxonomy that formally frames the sim-to-real techniques from key elements of the Markov Decision Process (State, Action, Transition, and Reward). Based on the framework, we cover comprehensive literature from the classic to the most advanced methods including the sim-to-real techniques empowered by foundation models, and we also discuss the specialties that are worth attention in different domains of sim-to-real problems. Then we summarize the formal evaluation process of sim-to-real performance with accessible code or benchmarks. The challenges and opportunities are also presented to encourage future exploration of this direction. We are actively maintaining a repository to include the most up-to-date sim-to-real research work to help domain researchers.

==> sections/domainRandom.tex <==
\subsection{Domain Randomization}




\subsubsection{State Representation}
Representation grounding (RG) is a technique focusing on the State element of the Markov Decision Process in which the agent’s observations are mapped to key characteristics of the environment to facilitate the learning process [?]. The primary objective of RG is to align the agent's observations with real-world phenomena, thereby addressing the Sim-to-Real gap. Notably, recent works focusing explicitly on bridging this gap through RG—such as [S2R VLN, Reduce S2R, Human Ambiguity, R2S2R, Manipulate Object Collections]—are comparatively fewer than those employing Domain Randomization.
\\

One noteworthy approach within RG is Visual-Representation Grounding (VRG) [Human Ambiguity, TransVG], wherein an agent seeks to segment locations described by natural language. The work presented in [Human Ambiguity] tackles the challenges associated with visual grounding by introducing a fully decoupled modular framework. This framework segments objects in crowded scenes based on natural language descriptions, effectively addressing the limitations of traditional methods. By utilizing scene graph annotations and training each module independently in simulation, it enables robust and interpretable visual grounding for service robots interacting with non-expert users. This modular approach not only enhances performance across diverse scenarios but also provides a clear pathway for bridging the Sim-to-Real gap in robotic applications. Conversely, [TransVG] proposes a transformer-based framework for VRG that efficiently associates language queries with relevant image regions. By reformulating visual grounding as a direct coordinates regression problem and leveraging a simple stack of transformer layers, it circumvents the complexities tied to traditional methods. Although [TransVG] does not explicitly address Sim-to-Real applications, it offers an alternative technique for visual grounding that complements the insights provided by [Human Ambiguity]. Additionally, [Reduce S2R] aims to minimize the Sim-to-Real gap by incorporating depth images into the agent's observations, grounding these observations in reality.
\\

RG is particularly prominent in a widely studied problem formulation known as Vision-Language Navigation (VLN), where an agent learns to ground language instructions to both visual observations and actions [S2R VLN]. Various methodologies for addressing representation grounding are employed within works that utilize the VLN problem formulation [S2R VLN, Scene Intuitive, Are You Looking?, S2S]. These diverse RG techniques in VLN may serve as inspiration for future research endeavors aimed at bridging the Sim-to-Real gap. For instance, [Scene Intuitive] exemplifies the integration of both VLN and VRG by enabling agents to localize target objects based on high-level natural language instructions. This work implements a two-stage training process that enhances cross-modal understanding and effectively links language with visual environments. In a similar vein, [S2R VLN] explores the challenge of transferring a VLN agent trained in simulation to a physical robot operating in an unseen environment. By employing a subgoal model, this study effectively bridges the gap between high-level discrete navigation commands and the robot's low-level continuous actions. It uniquely utilizes representation grounding by developing an occupancy map and navigation graph that align high-level language instructions with real-world navigation points, thereby facilitating the effective grounding of the robot's actions within its physical surroundings. Furthermore, [Are You Looking?] investigates how grounding language instructions—such as "turn right" and "stop at the door"—can be achieved through multiple modalities. This research reveals that models relying solely on geometric route structures can outperform those dependent on visual features in unseen environments, presenting a contrasting perspective to other works that underscore the significance of visual input for effective representation grounding. This highlights a potential avenue for future research in optimizing the balance between visual and structural modalities in VLN tasks. Lastly, recent research [S2S] comparing two VLN environmental paradigms, including the continuous VLN-CE setting, uncovers a significant performance gap, with agents struggling to transfer effectively from topological to continuous environments. This study emphasizes the necessity of refining transfer techniques to sustain performance across varying levels of realism, distinguishing itself from [Scene Intuitive] by focusing more on the challenges of sim-to-sim transfer rather than the direct grounding of language instructions.
\\

The remaining works discussed in this section each present distinct methodologies for addressing representation grounding, showcasing a diverse array of approaches that enrich the broader understanding of RG. While some of these studies may not directly target Sim-to-Real transfer, they provide valuable insights and techniques that could inspire future research in this domain. For instance, [Read watch move] introduces a reinforcement learning-based framework for video grounding, formulating the task as a sequential decision-making process that allows an agent to progressively regulate temporal grounding boundaries. Similarly, [TSP] focuses on temporally grounding language in untrimmed videos through a framework that mimics human decision-making, enabling iterative refinement of temporal boundaries while clearly representing semantic concepts as branches in the policy. More closely aligned with Sim-to-Real transfer, [R2S2R] grounds the environment by adopting a Real-to-Sim approach, which generates "digital twin" simulations from minimal real-world data. This methodology aids in grounding the representations in the simulation to the actual real-world environment and enhances policy robustness without extensive human oversight. Additionally, [Weakly-Supervised Phrase Grounding] expands on the concept of representation grounding by presenting a dual reinforcement learning framework that directly optimizes the phrase grounding model, effectively linking textual phrases to their corresponding image regions in a weakly-supervised context. This approach underscores the importance of establishing robust connections between language and visual representations—a central theme across the discussed works—highlighting the potential for integrated strategies that leverage both language and visual cues to enhance grounding performance. Finally, [Manipulate Object Collections] is directly related to Sim-to-Real transfer, proposing a method for sim-to-real robot learning that exploits simulator state information, allowing for scalability across numerous objects. This study trains two encoders on raw object pose targets to learn representations that accurately ground the state information of a multi-object environment. Their evaluations demonstrate that employing grounded state representations to train a reinforcement learning policy improves performance and contributes to bridging the Sim-to-Real gap.


==> sections/extra.tex <==

\section{Domain Randomization}
Domain randomization (DR) is a technique that targets the state element \textit{S} of the Markov Decision Process to bridge the ‘Sim-to-Real’ gap, enhancing model generalization by randomizing simulation parameters [28]. The core idea of domain randomization is to train models on extensive sets of randomized simulation data so that the real world appears as just another variant of these randomizations [28]. Due to its ease of implementation and capability to produce robust policies, DR has achieved remarkable success in bridging the “Sim-to-Real” gap. However, successful implementations often require expert-driven manual tuning of parameter distributions, making it a time-intensive process [Closing the loop]. This challenge raises several key questions: What data is needed to learn the parameter distribution? And how can the parameter distribution be learned? This challenge prompts several key questions: \textit{What data is needed to learn the parameter distribution}, and \textit{how can the parameter distribution be learned?} We will start by examining the data requirements for different methods (a breakdown is provided in the accompanying table), followed by a discussion on approaches to learning the parameter distribution.

\paragraph{What data is needed to learn the parameter distribution?}
To bypass the need for manually tuning parameter distributions, data can serve as a substitute for domain expertise. This data can be gathered in four main ways: using only the simulation, using pre-collected real-world data, using real-world policy rollouts, or using human demonstrations.

\begin{enumerate}
    \item The first strategy involves generating data solely through simulation to learn the parameter distribution. This approach is advantageous as it requires no additional information beyond the default simulation environment settings. However, DR may achieve better results when supplemented with real-world or human demonstration data, as these sources are more likely to reflect the target domain.
    \item The second approach uses pre-collected real-world data, which closely aligns the parameter distribution with that of the target domain. However, this method depends on access to real-world data, which may be limited, or requires direct access to the physical system, which isn’t always feasible.
    \item If ongoing access to the real-world physical system is available, the third approach—using real-world policy rollouts to learn the parameter distribution—can be effective. The benefit here is the ability to update the parameter distribution dynamically during training. However, the drawback is the continuous need for physical system access, which may not always be possible.
    \item Lastly, human demonstrations can be utilized to learn the parameter distribution. Rather than fine-tuning simulation parameters, a single human demonstration can provide expert data to set the distribution for DR. The limitation is that some tasks do not allow for human demonstration, rendering this strategy inapplicable.
\end{enumerate}


\paragraph{How can the parameter distribution be learned?}
Various methods are available for learning the parameter distribution in DR, and the choice of method often depends on data availability. If extensive real-world expert data is accessible, it is generally preferred over methods relying solely on simulation data. The most widely adopted approach involves statistical methods, though other techniques—such as adversarial environment generation and gradually expanding the parameter distribution—are also utilized. We will first discuss the statistical methods followed by other approaches to learning the parameter distribution.

\begin{enumerate}
  \item Statistical methods are commonly used for learning the parameter distribution, including Bayesian optimization [BayRn], KL-divergence constraints [Closing Loop], Covariance Matrix Adaptation Evolution Strategy [DROID], likelihood-based approaches [DROPO, Soft Robots], Elastic Weight Consolidation [Continual DR], and a likelihood-free inference method [BayesSim]. For example, Bayesian optimization [BayRn] adapts the domain parameter distribution during training, allowing for efficient policy optimization with minimal prior domain knowledge. Another approach [Closing Loop] uses an iterative KL-divergence constraint to refine the simulation parameter distribution, improving policy transfer with minimal real-world rollouts. Similarly, [DROID] formulates domain randomization as a distribution optimization task, using Covariance Matrix Adaptation Evolution Strategy (CMA-ES) and human demonstrations to improve policy transfer across tasks. Additionally, [DROPO] applies a likelihood-based approach to model parameter uncertainty using a limited offline dataset, enhancing sim-to-real transfer without extensive real-world interactions. [Soft Robots] builds on [DROPO] by retaining the likelihood-based approach while adapting it to partially observable environments. In a different approach, [Continual DR] combines domain randomization with continual learning, using Proximal Policy Optimization (PPO) [?] and Elastic Weight Consolidation (EWC) [?] to evaluate neural network parameters. Lastly, [BayesSim] offers a framework for handling simulation parameter uncertainty through likelihood-free inference, enhancing DR strategies by deriving posterior distributions from simulation outputs and real-world trajectories.
  \item Many other approaches exist for learning the parameter distribution which do not center on statistical methods. [MARL UAV] and [SSR Active DR] both use some form of generative learning to learn the parameter distribution. [MARL UAV] uses a nature player as the adversary to generate more difficult environments for the agents. In contrast [SSR Active DR] pits two agents Alice and Bob against each other to co-evolve a goal curriculum and generate a self-supervised reward to use for evolving the environment curriculum. This work builds upon [Active DR] which uses a reference environment (default simulation) and DR generated simulation instances to learn a discriminator that learns to generate the reward in place of the self-supervised piece above. In both [SSR Active DR] and [Active DR], the idea to grow the environment towards agent difficulty remains the same. Another work which builds an environment curriculum during learning is [Rubik’s Cube], which progressively increases randomization in the environment as the agent is able to meet desired performance thresholds. The general idea remains the same across these works, demonstrating impressive performance by focusing on shifting the DR distribution towards areas of difficulty for the agent. Instead of building a curriculum of environments, [Efficient S2R] adopts a hybrid approach. They accept the challenge of a potentially too narrow DR distribution, but overcome this challenge using domain adaptation with real-world rollouts after DR has been applied. This work demonstrates the effectiveness of combining domain randomization with another sim-to-real technique, showcasing the potential effectiveness of hybrid DR approaches. Lastly, [Cyclical PD] focuses on splitting the ranges of randomized parameters into sub-domains to learn local policies for each, finally distilling the local policies into a global policy for sim-to-real transfer. This work provides a way to utilize large randomization ranges for DR, ensuring that the parameter distribution encapsulates the target domain which improves sim-to-real transfer.
\end{enumerate}

\begin{table*}[t]
    \centering
    \begin{tabular}{|p{5cm}|c|c|c|c|}
        \hline
        \textbf{References} & \textbf{Data} & \textbf{Statistical Methods} & \textbf{Generative} & \textbf{Other} \\ \hline
        [Active DR] & Simulation only && \checkmark & \\ \hline
        [SSR Active DR **] & Simulation only && \checkmark & \\ \hline
        [Rubik’s Cube **] & Simulation only && \checkmark & \\ \hline
        [Efficient S2R **] & Simulation only & & & \checkmark \\ \hline
        [MARL UAV] & Simulation only & & \checkmark & \\ \hline
        [Cyclical PD] & Simulation only & \checkmark & & \\ \hline
        [Continual DR] & Simulation only & \checkmark & & \\ \hline
        [DROPO] & Real-world data (pre-collected) & \checkmark && \\ \hline
        [Soft Robots] & Real-world data (pre-collected) & \checkmark && \\ \hline
        [BayesSim] & Real-world data (pre-collected) & \checkmark & & \\ \hline
        [Data Efficient] & Real-world policy rollouts & \checkmark & & \\ \hline
        [Closing Loop] & Real-world policy rollouts & \checkmark && \\ \hline
        [DROID] & Human demonstration & \checkmark && \\ \hline
        [DROPO ** repeat can use human demo] & Human demonstration & & \checkmark & \\ \hline
    \end{tabular}
    \caption{Summary of data sources and methodological approaches for domain randomization (DR) references. Simulation-only methods rely exclusively on simulations. Real-world data methods use precollected real data. Real-world policy rollouts involve real-world policies, and human demonstration methods may utilize or require human demonstrations for DR. Statistical Methods, Generative, and Other columns indicate the use of statistical, generative, or other relevant techniques.}
\end{table*}

